Data Sanity Check for Deep Learning Systems via Learnt Assertions

Reliability is a critical consideration to DL-based systems. But the statistical nature of DL makes it quite vulnerable to invalid inputs, i.e., those cases that are not considered in the training phase of a DL model. This paper proposes to perform data sanity check to identify invalid inputs, so as to enhance the reliability of DL-based systems. We design and implement a tool to detect behavior deviation of a DL model when processing an input case. This tool extracts the data flow footprints and conducts an assertion-based validation mechanism. The assertions are built automatically, which are specifically-tailored for DL model data flow analysis. Our experiments conducted with real-world scenarios demonstrate that such an assertion-based data sanity check mechanism is effective in identifying invalid input cases.

==> tex/figs/fig1.tex <==
\begin{figure*}
    \subfigure[Valid inputs and normal workflow]{

        \includegraphics[width=0.72\linewidth]{pic/TrafficMotivationNormal.png}
        \label{fig:side:traffic_normal}
    }
    \subfigure[Invalid input and misbehavior]{

        \includegraphics[width=0.25\linewidth]{pic/TrafficAbnormal.png} 
        \label{fig:side:traffic_abnormal}

    }
    \caption{Motivating examples for a traffic sign recognition system}
     \label{fig:traffic_motivate}
\end{figure*} 

\begin{figure}[htbp]
	\centering
	\subfigure[Target categories in the training set of Fashion-MNIST]{
		\includegraphics[width=0.9\linewidth]{pic/show_fashion_mnist.png}
		\label{fig:moti:show_fashion_mnist}
	}
	\subfigure[Invalid inputs that appear in the testing set of Fashion-MNIST]{
		\includegraphics[width=0.9\linewidth]{pic/show_mnist.png} 
		\label{fig:moti:show_mnist}
	}
	\caption{Examples of invalid inputs in a properly fetched public dataset}
	\label{fig:show_fashionmnist}
\end{figure}


==> tex/intro.tex <==

\section{Introduction}

% 神经网络好用，用来做系统，用在critical的地方，可靠性很重要
Deep learning (DL) techniques have shown their effectiveness in various application areas \cite{DBLP:conf/iccais/DuanM15, DBLP:journals/tmi/GreenspanGS16, DBLP:conf/kbse/AbdessalemNBS16}, even in safety-critical scenarios\cite{DBLP:journals/corr/BittelKTT15, DBLP:conf/cvpr/KimP17, DBLP:conf/ijcnn/SermanetL11}. Image recognition module for auto-driving vehicles \cite{DBLP:conf/iccais/DuanM15, DBLP:conf/cvpr/KimP17}, for instance, determines what operation should be taken based on the real-time images captured by cameras. In such safety-critical scenarios, any unreliable system misbehavior may cause severe incidents. Reliability is hence of great significance to practical DL-based systems.

% 高可靠性很重要，需要系统可以处理任何输入，但现实中输入不保证合理, 现实中不在合法输入域中的输入会损害系统可靠性

Recently, extensive efforts in the software community have been put in addressing the reliability concern of DL-based  systems \cite{DBLP:conf/issre/MaZSXLJXLLZW18, DBLP:conf/kbse/SunWRHKK18,DBLP:conf/kbse/ZhangZZ0K18, DBLP:conf/sosp/PeiCYJ17,DBLP:conf/icse/TianPJR18}, focusing on in-house approaches, {\em e.g}., testing. These approaches attempt to build a robust DL model that is expected to achieve high accuracy in real deployment. But before they become mature solutions, reliability still remain a critical concern towards the wide application of DL  systems in safety-critical scenarios.

Unlike this line of research, this work aims at improve reliability during system runtime via input verification. 
We note that the statistical-inference nature of DL makes it quite vulnerable to invalid inputs. Those unexpected types of input data which are not considered in the training phase of a DL model can mislead the model to wrong outputs. A good sanity check of inputs is hence critical in avoiding misbehavior of DL-based systems.

Sanity check is not a new idea to the software community. It is widely-accepted that every software system has its valid input domain \cite{white1980domain, DBLP:conf/kbse/TanejaLMXT10, li2010perturbation, DBLP:conf/issta/TsankovDB13 }. Inputs in such a domain, namely, {\em valid} inputs, are expected to receive  proper execution results.
Unfortunately, in real circumstances, there is no guarantee that the inputs are always valid.   
Anomalous, unexpected inputs may arrive and result in unpredictable misbehavior, which in turn degrades reliability. 

For DL-based systems, take a classification task for example. A DL model is trained based on the cases belonging to a set of target categories ({\em e.g.}, different traffic signs for a traffic sign recognition system\cite{DBLP:conf/ijcnn/SermanetL11}).
The cases in such target categories form the valid input domain.
But in real practice, other cases belonging to extra categories may be taken as inputs. 
Without a proper checking, even a sophisticated DL model will process an invalid case and generate classification result, indicating that the case belongs to one of the target categories ({\em i.e.}, a traffic sign).
This result is obviously wrong, which may potentially incur risks.
Suppose a traffic sign recognition system in an auto-driving vehicle receives a commercial logo by the street as an input. If it is mistakenly classified as a certain traffic sign, the operations of auto-driving vehicle taken accordingly may lead to severe accidents. Hence, it is critical to develop a mechanism for DL-based systems that can detect invalid inputs, so as to enhance its reliability. 


% A deep learning systems is usually developed following a clearly-defined requirement. {\em e.g.}, for a classification system, the requirement specification should stipulate the categories that this system should classify. Thereby it's model structure and training data are carefully selected accordingly. Hence, these pre-defined categories constrain the valid input domain of of the system, leaving no capability for it to handle untrained classes. However, such invalid inputs do come about after the system's deployment in the wild. For instance, the traffic sign recognition system will come across commercial logos on the street side, and take it as input and mistakenly classify it as a certain type of traffic sign. Such classification result can lead to severe safety incidents if no exceptions are raised. Therefore, it is vital to develop a mechanism for deep learning systems that enhance its reliability by detecting invalid inputs({\em i.e.} untrained data class), so as to prevent potential risks. 

%Consider a three-class classifier recognizing traffic signs used in auto-driving system, as shown in Figure \ref{XXX}. The model structure determines that only the result for three classes will be given, and the training data determines that the system only targets on classifying the three signs on the left, which forms the valid input domain. However, one may come across a sign on the right in practice, while the system will still take it as input and give a classification result. Since such data has never been used during training phase, the given result can be unpredictably chosen among the three classes. The given example shows the case where classification result turns out to be an entirely different direction opposite to what the invalid input should be, and accordingly huge potential danger would appear in consequence. Hence, when regarding untrained classes as invalid inputs, they can cause severe risks by giving unexpected results.
 
%Instantly, we can use the output of the DL model, .
 
%Detecting invalid inputs is similar to the problem of obtaining the result certainty produced by a DL model, 
%Since avoiding risks from invalid inputs in system runtime is a crucial task, it has received much attention in both software engineering and machine learning communities. From a software testing perspective, some suggest that manipulated corner cases of DL models should be found with an SVM-based validation \cite{wu2019deepvalidation}. Machine learning researchers regard detecting invalid inputs as the problem of obtaining the result certainty produced by a DL model. 
%So model weights, dropout, and logits are considered as indicators of result certainty to some extent \cite{hendrycks2016baseline, DBLP:conf/icml/GalG16, DBLP:conf/nips/Lakshminarayanan17}. 
%Moreover, one can consider to include an additional class in the model that indicates an input is not in the target categories \cite{bendale2016towards, scheirer2013toward}. 
%However, these approaches generally require an exhaustive retraining of a DL model and may even degrade its original accuracy, not to mention the runtime overhead incurred. As a result, they cannot be applied to existing models. Moreover, it typically requires heavy machine learning expertise of to apply them, hindering their wide application in DL application domain.   

Detecting invalid inputs is similar to the problem of obtaining the result certainty produced by a DL model, which has received much attention among existed work. 
Model weights, dropout, and logits, are considered as indicators of result   certainty to some extent \cite{hendrycks2016baseline, DBLP:conf/icml/GalG16, DBLP:conf/nips/Lakshminarayanan17}. 
Some suggest that manipulated corner cases of DL models be detected with an SVM-based validation \cite{wu2019deepvalidation}.  
Moreover, one can consider to include an additional class in the model that indicates an input is not in the target categories \cite{bendale2016towards, scheirer2013toward}. 
However, these approaches generally require an exhaustive retraining of a DL model and may even degrade its original accuracy, not to mention the runtime overhead incurred. As a result, they cannot be applied to existing models.

Moreover, it typically requires heavy machine learning expertise of to apply those complicated approaches, hindering their wide application in DL application domain. 
%To provide an efficient and easy-to-use approach from a software perspective
In this paper, we present \textbf{\deep}, a data sanity checking framework that provides systematic data \textbf{San}ity ch\textbf{e}ck for \textbf{D}eep \textbf{L}earning-based Systems.
%Existing work exhibits the attempt on using SVM to validate \cite{wu2019deepvalidation}. But we find that the approach proposed can't achieve satisfactory effect in our scenario.
%Some works from DL community also discuss their analysis on model weights, dropout, and logits, which to some extent indicate the certainty of the result\cite{hendrycks2016baseline, DBLP:conf/icml/GalG16, DBLP:conf/nips/Lakshminarayanan17}
%However, these solutions require DL system maintainers to obtain specific expert knowledge towards the subtle details of the model. This can be a great obstacle for inexperienced maintainers or users to adapt these approaches to different tasks.
%However, the requirement on specific expert knowledge towards the subtle details of the model forms a great obstacle for inexperienced maintainers or users to adapt these approaches to different tasks.
%Moreover, one can include an additional class that indicates an input is not in the target categories, {\em i.e.}, it is an invalid input\cite{bendale2016towards, scheirer2013toward}. But adding an extra class needs an entire rework on the training phase, which is rather costly to be applied on a settled model, and may also negatively influence the original accuracy. To provide an efficient and easy-to-use solution from a software perspective, in this paper we propose \textbf{\deep}, a white-box verification framework that provides systematic data \textbf{San}ity ch\textbf{e}ck for \textbf{D}eep \textbf{L}earning-based Systems.
\deep\ serves as a lightweight, flexible, and adaptive plugin for DL models, which can achieve effective detection of invalid inputs during system runtime. %Such detection has to conquer the uninterpretable computation process of deep learning system, so as to seek for differences on between valid and invalid inputs from the system perspective. In addition, in order to retain the system performance, it is also required that the approach should not negatively affect the original classification accuracy on valid inputs. And lastly, for the efficiency concern, the extra computation cost ought to be minimized.
% data sanity check因此很重要，我们设计了工具来实现。但是工具需要在不可解释的深度学习过程中寻找合法与非法输入的差异，并且不影响模型的原有效果，以及高效。
The key consideration of the \deep design is that a DL-model will behave differently when given valid input cases and given the invalid ones. Following the classic notion that behavior deviation is an important symptom of bugs \cite{engler2001bugs}, we identify invalid input cases via examining the 
behavior deviation. 

Since a DL model is not complicated in its control flow, we use data flow to model its behaviors. 
Specifically, \deep\ provides an assertion-based mechanism, which can insert a set of automatically-built assertions between different layers in a neural network.
%Via a light, automatic instrumentation to the target network, \deep\ extracts the data flow footprints. It then processes the footprints with an assertion-based mechanism. 
Such specific-tailored assertions are constructed via Auto-Encoder (AE)\cite{hinton2006reducing}, which reconstructs the intermediate results of the model, and evaluate the data flow deviation with the reconstruction loss. As both the structures and weights of the AEs are automatically set and trained, \deep\ achieves an effective and efficient detection on invalid inputs with minor human efforts and expertise. Moreover, such AE-based assertion mechanism exhibits a perfect compatibility with the DL model. Consequently, \deep\ is a non-intrusive solution, which enhance DL model reliability, while keeping it's original accuracy.
%Similarly to traditional assertions for general programs inserted between code blocks, the assertions are inserted in certain network layers, so as to detect behavior deviations in a data flow perspective.  


%One remarkable progress of our work is that we are focusing on real-world cases which may actually come about in practical use. Existing works that apply software engineering domain knowledge in optimizing deep learning systems only consider samples that are manipulated from original practical cases\cite{XXX}. We indicate that our reality-oriented approach reveals more practical significance. Our evaluations on raw real-world cases demonstrate that our approach achieves very satisfactory results in detecting realistic invalid inputs, and therefore protects deep learning systems from potential risks.

We summarize the contributions of this paper as follows. 

\begin{itemize}
    \item We approach reliability enhancement of DL systems via data sanity check. We proposed a verification framework, namely \deep, to perform data sanity check for DL-based systems. \deep\ provides AE-based assertion mechanism to detect data flow deviation of DL models. The automatic generation of AEs within the assertions makes \deep\ an effective, efficient and easy-to-use tool to identify invalid input cases for DL 
    systems.
    %\deep\ is an assertion-based approach, where the assertions are automatically learned and inserted. 
    To our knowledge, \deep\ is the first verification framework based on assertions that enables additional protections against invalid input cases for DL systems. Our work can shed light to other practices in improving DL reliability.
    \item \deep\ adopts a non-intrusive design that will not degrade the performance of the target DL model. In other words, the \deep\ mechanism does not require to redesign the target dl model. As a result, \deep\ can be easily applied to existing DL-based systems.
    \item We show the effectiveness and efficiency of invalid input detection via real-world invalid input cases, other than manipulated faulty samples typically used in the community. This proves the \deep\ mechanism is promising. In addition, our experimental method may shed light to other DL tool evaluation work in the software engineering community. 
\end{itemize}
    
We organize the rest of the paper as follows. Section 2 introduces the preliminary knowledge of this work. In Section 3, we discuss the motivations and challenges. Sections 4 elaborates the \deep\ design in detail. We present our experimental results with real-world case studies in Section 5 to evaluate our tool effectiveness. The related work is introduced in Section 6. Section 7 provides further discussions and we conclude the paper in Section 8.


==> tex/moti.tex <==




\section{Problem Statement} \label{sec:motivation}



%输入数据需要和训练数据同类，不是同类的数据会被强行分类成一个结果，这个结果会导致危险后果
%As we have discussed
A DNN model is trained with a set of training data samples. A developer will typically use representative samples that will be encountered in real deployment to train the DNN model. In other words, she expects that the input samples in real deployment fall in the same  categories with training samples. For example, a model to recognize flowers can only recognize flowers, but not animals. To facilitate our discussions, we call the expected samples the {\em valid inputs}, the unexpected samples belonging to different categories the {\em invalid inputs}.

Unfortunately, when deployed in production environment, a DNN model will inevitably meet invalid inputs. 
However, current DNN design practice generally does not consider the existence of invalid inputs. As a result, even a sophisticated DNN model may make obvious mistakes. For example, a DNN model to recognize flowers may consider a dog as a sunflower. 


Lack of sanity check of input data may result in severe consequences in safety-critical applications. Let us consider a traffic sign recognition DNN model in auto-driving vehicles\cite{DBLP:conf/ijcnn/SermanetL11}. 
Figure \ref{fig:side:traffic_normal} shows its normal workflow when valid traffic signs are given as inputs. 
Even if the DNN model can recognize traffic signs perfectly by classifying traffic signs to the correct classes, it may produce severe errors.   
For example, sometimes a commercial logo on the roadside will be fed into the DNN model, as shown in Figure \ref{fig:side:traffic_abnormal}. If without a sanity check of inputs, the DNN model will produce a classification result accordingly. In other words, it will mistakenly recognize the logo as a specific traffic sign.
The auto-driving vehicle may potentially suffer an accident.

%这种非法输入的现象很普遍，在学术研究中，keras下载的fashion mnist数据集的测试集中混合了mnist的数据，导致实验准确率下降，并且难以发



Encountering invalid inputs is not just illusive cases. 
Some public datasets widely used in deep learning studies do contain obviously-invalid samples, {\em i.e.}, those totally irrelevant to the training samples. For example, the Fashion-MNIST\cite{xiao2017fashion} dataset provided by version 2.1.6 of Keras, a widely-used DNN development tool\cite{chollet2015keras}, mistakenly contains samples that should belong to the MNIST\cite{DBLP:journals/spm/Deng12} dataset in its testing set\footnote{Fashion-MNIST is a public dataset providing pictures of fashionable clothing. MNIST is another public dataset consists of handwritten digits images.}. We show such a case in Figure \ref{fig:show_fashionmnist}.
With invalid samples during model testing, a DNN model will produce errors and show poor performance in accuracy. However, even for the in-house data, it is quite labor-intensive to pinpoint the existence of the invalid samples manually, not to mention the localization of invalid samples that may met in real deployment.  

%希望实现对系统异常输入有一个预警，抛出异常

Therefore, an effective sanity check mechanism of input data is highly critical to improve the reliability of a DNN model. Such a mechanism can automatically detect if a given input is invalid. Follow-up approaches are then possible to minimize the influence of the invalid inputs. For example, manual operation can be enforced to override DNN decisions. The aim of this work is to provide our experience in designing such a sanity check framework, namely, \deep.  

However, although a sanity check mechanism of input data is of great importance to the reliability of DNN-based software, designing such a mechanism is not an easy task. The features of DNN introduce many specific difficulties to data sanity check. We present several challenges faced by such a sanity check as follows.

%\subsubsection{Uninterpretable computing process of DNN}
First of all, state of the art still lacks a good interpretation on how on earth a DNN works. For example, why a neuron in a DNN is activated and what its subtle role is in the whole task. 
A set of inputs may share the same classification result, while the computation processes through the network vary from case to case. 
Without an accurate understanding of how a DNN works, it is very difficult to build a principle based on the execution dynamics to examine the validity of the input data. 


%\subsubsection{Non-intrusive data sanity check}
%需要保持模型原有的效果，非侵入式
%A straight-forward solution for the data sanity check problem in deep learning is to reconstruct a new model which adds those extra invalid data as an additional class to be classified. 
Secondly, Data sanity check is in nature an additional supportive component, which must not influence the original DNN model performance on valid inputs.
The DL system's performance relies heavily on the preset network structure and trained parameters. Any slight changes among these components can greatly affect the performance. 
%However, a DNN model generally requires a computation-intensive training phase before it can be applied in practice. 
%The final system performance relies heavily on the preset network structure, hyper-parameters, and training data. Any slight changes among these components can greatly affect the performance. 
Hence, it is required that such data sanity check should be a carefully-designed mechanism which works in a non-intrusive manner. Straight-forward approaches like model reconstruction fail to achieve satisfaction. 
%Instead, \deep\ successfully leverages the post-training intermediate data from the network to reach the goal. It proves to be a useful and side-effect-free tool for deep learning system.


%\subsubsection{Low computation overhead}
%需要低开销的完成异常输入检测
Last but not least, it's worth noting that the mechanism of data sanity check usually turns out to be a set of very brief inspections, rather than a more exhaustive round of redundant testing. As many DL-based systems are deployed to handle real-time tasks, the additional sanity check on the input data should be accomplished with a low computation overhead. Hence, we expect a cost-efficient tool to perform such process. %Accordingly, \deep\ introduces compatible solution to deep neural network via AutoEncoders, which can easily adapt to a pre-trained network as a lightweight plugin. An efficient verification process is thereby achieved with a low computation overhead.

We will elaborate how \deep's special design helps in handling these challenges in the next section. 

%\subsection{Availability in real world cases}



==> tex/new_method.tex <==
\section{Methodologies}

In this section, we will introduce the design of \deep. We first show the overview of \deep and then watch into its technical details. 

\subsection{Overview}\label{overview}

Figure \ref{fig:overview} shows the framework of \deep. Generally, for a pre-trained DNN model, the execution process of \deep\ follows the workflow as below: First, a series of AE-based assertions are inserted into the structure of a settled DNN. The underlying AEs of these assertions are automatically pre-trained using the intermediate data produced by the training set ({\em i.e.} a set of valid inputs) of the DNN model. For a given input in real practice, such assertions take the intermediate data of DNN as inputs to evaluate the anomalous degree via the reconstruction losses. We check each assertions by using properly preset thresholds to constrain the losses. The assertion results then determine the validity of given input.  

\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.9\linewidth]{pic/Overview.png}  
	\caption{Overview of \deep} 
	\label{fig:overview}  
\end{figure*}
%strategy, which respectively mean aborting immediately whenever assertions fails, or giving an overall judgement via all assertion results. 

% It's worth noting that \deep\ is designed in a white-box manner, which considers a deep neural network as a sequential iterative program. According to the previous introduction in Section II, we concluded the computation process of neural network as the following functional expressions, having x as the input data, $f_{1..n}$ as the connection functions, $a_{1..n}$ as the activation functions, and ${NN}_{1..n}$ as the output for each layer.

% $$
% \begin{matrix}
% {NN}_{1} = a_{1}(f_{1}(x)) \\ 
% {NN}_{2} = a_{2}(f_{2}({NN}_{1})) \\
% ... \\
% {NN}_{n} = a_{n}(f_{n}({NN}_{n}))

% \end{matrix}
% $$

% In this case, it provides the possibility to retrieve the intermediate results({\em i.e.} ${NN}_{1..{n-1}}$) from the computation dataflow of the network. 
Similar to checking runtime internal states in conventional program testing, we focus on analyzing such intermediate data to discover the abnormal behavior of neural network. Specifically, our working process is built on the belief that the intermediate data of valid inputs and invalid inputs follow different distribution. We will then describe the details on how we evaluate such differences to indicate invalid inputs. 

\subsection{Auto-Encoder based Assertions}

For conventional software, developers typically use assertions to check whether the system runtime satisfies certain conditions. Similarly, \deep\ provides the assertion mechanism to inspect the runtime internal states for DL based systems. Such assertions set constrain on the intermediate result of certain layers in the DNN to identify model's deviate behaviors.

We introduce AE in \deep\ to build the assertions. As previously described, data in a certain pre-trained  distribution can successfully be restored by AE at a low loss. Hence we take advantage of this nature to assert if the intermediate data of the target DNN deviate from the distribution produced by the valid inputs. Specifically, given a pre-trained neural network $N$, one can insert assertions based on AE between its layers.
These AEs are automatically generated by the \deep\ framework, which requires little manual effort to conduct exhaustive fine-tuning. We conclude the automatic generation process from two aspect:
\begin{itemize}
    \item {\textbf Weights training}: The AEs have to be properly trained so as to form their reconstruction capability towards the distribution of intermediate data produced by valid inputs. Intuitively, the training set, on which the target model is trained, always serves as a standard of valid input. Therefore we consider the training set of $N$ as a large accessible set of valid data. \deep\ feeds the training data into $N$ and extracts the intermediate data flow processed by the layer where assertions are inserted. These extracted data are then used to train the corresponding AEs. With such automatic training process, these AEs fit the distribution of the intermediate data from valid inputs, and are expected to properly restore the intermediate data if valid inputs are given to $N$.

    \item {\textbf Structure construction}: The structure of the AEs can be automatically determined according to the shape of intermediate data. %Fig \ref{fig:XXX} shows an example on how the structure of an AE is constructed when inserted at a certain layer. 
    Specifically, the input dimension and the output dimension are set to the same as the size of the corresponding intermediate data. For the encoding phase of AE, the number of neurons is cut in half layer by layer. And correspondingly, the number of neurons in the decoding phase doubles layer by layer, so as to match the symmetric structure. We suggest the number of the layers should be neither too deep to compute efficiently, nor too shallow to perform the restoration properly. A default depth is set to 5 in \deep, which is a proper value in practice for inexperienced users to apply directly, as well as supporting a customization for expert users.%In our practice, we defaultly set the number of layers as 5, which is neither too deep to compute efficiently, nor too shallow to perform the restoration properly.  
\end{itemize}

These AEs are then used to perform assertion check for the intermediate data. Algorithm \ref{alg:assert} formally concludes the checking process of a single inserted assertion. The output of the layer where the assertion is inserted is taken as the input for it's underlying AE. AE process the input and give a reconstruction result. An MSE loss is then calculated with the input and the reconstruction result. As a high MSE loss indicates the improper reconstruction, we will further set the constrain by giving a certain threshold on the loss. The loss above the threshold reveals the assertion failures, which further indicates the invalidity of input. 
%For invalid inputs, the reconstruction leads to a huge deviation with a high loss value for the intermediate results of invalid inputs show abnormal patterns that don’t fit the AEs. 
%In practice, for every input fed to $N$, both the model output and the MSE loss for every inserted AE are calculated simultaneously.



Particularly, we demonstrate the reasons for choosing AE as the essential module for the assertion mechanism of \deep. First, AE is an unsupervised approach, which can effectively identify data anomalies by transfering it into intuitionistic deviate behaviors ({\em i.e.} failing to perform restoration). Rather than understanding the feature pattern in intermediate data according to exhaustive extra labelling on valid and invalid inputs, AE turns out to be a more feasible solution that evaluates the deviation with certain behaviors. AE provides an access to the anomalous degree of internal states via the reconstruction performance, which helps to achieve a better sanity checking effect. 

Second, AE presents a high compatibility with the DNN model. Given that AE is a neural network itself, it can be perfectly inserted between layers of a target DNN model. Such nature enables \deep\ to provide the framework which supports flexible insertion of assertions. Therefore, AE is a  well-fitted extension for deep neural network to achieve additional functionalities.

Third, AE introduces low computation overhead in practice. Due to the conciseness of its structure, AE can be pre-trained and executed at a very low time cost with GPUs. We compared AE with several other mechanisms that can also be used in such scenarios. Results show that AE achieves the best efficiency performance.

In conclusion, from a software engineering perspective, the inserted AEs work as the assertions, so as to ensure the system's intermediate results follow a certain set of constrains. Invalid inputs are likely to break such constrains by generating abnormal intermediate results that AEs fail to reconstruct. Along with its good compatibility and cost-efficiency, we prove that such AE-based assertion is a effective approach to achieve data sanity check.

\begin{algorithm}[htbp]
	\caption{Assertion Check}
	\label{alg:assert}
	\begin{algorithmic}[1]
		\Require the intermediate result given by the layer where assertion inserted $ir$, the assertion's underlying AutoEncoder $AE$, preset threshold thres
		\Ensure a boolean value $ar$ represents the assertion result, {\em i.e.} pass or fail
		\Function{Assertion\_Check}{$ir$, $AE$, $thres$}
            \State // get the reconstructed vector $rv$ for $ir$ using $AE$
    		\State $rv := AE(ir)$
    		\State // compute MSE loss between $ir$ and $rv$ as the reconstruction loss
    		\State $loss := MSE(ir, rv)$
    		\State // check if loss exceeds the threshold
    		\If{$loss > thres$}
    		    \State // if so, assertion failed
    			\State $ar := \mathbf{False}$
    		\Else
    		    \State // otherwise, it passed
    		    \State $ar := \mathbf{True}$
    		\EndIf
    		\State \Return{$ar$}
    	\EndFunction
	\end{algorithmic}
\end{algorithm}

\subsection{Threshold Setting and Validity Verification}
%想要尽可能减少validation这个词的使用， 避免和徐辉DeepValidation太像
With assertions inserted, we further introduce how we select appropriate thresholds for each assertion, as well as how we verify the inputs validity according to the assertion results. 


\subsubsection{Threshold setting}
%An AE-based assertion evaluate the deviation of corresponding intermediate result with its reconstruction loss. The larger the loss value is, the more likely the input is abnormal. To conduct the assertion, a proper threshold should be set, which shows the upper bound of the normal reconstruction loss. As the design philosophy of \deep\ is to exploit the differences between valid and invalid input via intermediate results, we choose to set the thresholds, we set threshold according to the mean value of the reconstruction loss of all valid inputs. Formally, it can be expressed as the following equation:
To achieve an accurate detection on invalid input, it is vital to set proper thresholds on each assertion that constrain the valid upper bound of coresponding losses. As the design philosophy of \deep\ is to exploit the differences between valid and invalid input via intermediate results, we choose to set the thresholds as relative values with losses generated by the intermediate results of valid inputs. For a certain assertion, we calculate the mean loss by feeding the underlying AE with the intermediate result of training data({\em i.e.} the available valid inputs). And then the threshold is set at a relative scale towards such mean loss. Formally, it can be expressed as the follow equation:
$$
Thres = \delta \cdot \frac{\sum_{j=1}^{m} Loss_{AE}(IR_{j})}{m}
$$
The $IR_{j}$ stands for the input of the AE, which is the intermediate result at certain layer of the $j$th case in the training set. The $m$ means the total samples of the training set. The $\delta$  represents the scale coefficient, which determines the assertion threshold as a certain scale of the mean loss of valid inputs. 

Instead of setting different values of $\delta$ for different assertions, through practice, we find that a properly single value of $\delta$ works good enough to conduct input sanity check. Therefore, we only need to preset a proper $\delta$ rather than exhaustively fine-tuning series of values. Such selection strategy can be adjusted according to different scenarios. 
Usually, selecting a larger $\delta$ can detect more real invalid inputs but may mistakenly reject some valid inputs as well, while selecting a low $\delta$ tends to stay cautious in verifying inputs as invalid and may miss some true invalid cases. 
Our practice shows that selecting this scale coefficient in a interval from 2 to 4 ({\em i.e.} $\delta \in \left [ 2, 4 \right ]$) results in good performance.

	


\subsubsection{Validity Verification}


After receiving the result of each assertion, a proper judgement on the input's validity would be performed accordingly. In traditional software testing, it is common that a program aborts and raises exceptions once assertion failure occurs. Similarly, \deep's working process also follows such notion. In practice, for every input fed to the target DNN model, both the model output and the MSE loss for every inserted AE are calculated simultaneously. If any AE gets the reconstruction loss that exceeds the corresponding threshold, the assertion then fails and detects such input as an invalid case.  



We illustrate the input validity verification process at Algorithm \ref{alg:Validity Verification}. 
Specifically, when an input is given to the target DNN with assertion inserted, \deep\ extracts the intermediate data flow of the DNN and conduct checking process on every assertion according to Algorithm \ref{alg:assert}. 
%for every assertion $A_{i}$, we feed the output of the layer where it is inserted to its underlying $AE_{i}$, if the reconstruction loss $L_{i}$ generated from $AE_{i}$ is larger than the preset threshold, then the assertion $A_{i}$ claims failure, and \deep\ will raise exception to indicate that this input case is invalid. 
Only those inputs that pass all the assertions are verified as valid inputs that the DL system can properly handle. Such mechanism guarantees that for a given input, the dataflow of the DNN should always follow the pre-trained feature pattern throughout its computation process. This conforms the concept of reliability enhancement in conventional software testing, which requires the every sub-process of a software works as pre-defined requirements.

\begin{algorithm}[htbp]
	\caption{Input Validity Verification}
	\label{alg:Validity Verification}
	\begin{algorithmic}[1]
		\Require the intermediate results of a test sample $\mathbf{ir}$, a series of AutoEncoders $\mathbf{AE}$, the index list of layers where assertions inserted $\mathbf{SL}$, a series of preset threshold $\mathbf{thres}$
		\Ensure a boolean value $validity$ which means whether the sample is anomaly or not
        \State // default validity set to True 
		\State $validity := \mathbf{True}$
		\For{$\mathbf{each}\ i \in \mathbf{SL}$}
			\State // check the corresponding assertion inserted at $layer_{i}$
			\If{$\mathbf{not}\ Assertion\_Check(ir_{i},\ AE_{i},\ thres_{i})$}
			    \State // if assertion failed, set validity to False 
				\State $validity := \mathbf{False}$
				\State $\mathbf{break}$
			\EndIf
		\EndFor
	\end{algorithmic}
\end{algorithm}	

\subsection{Layer Selection}

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.95\linewidth]{pic/CNN.png} 
	\caption{A sample structure of CNN}
	\label{fig:method:CNN}
\end{figure}

In this part, we suggest some guidance for users to make choice on layers to insert the assertions. 
The implementation of \deep\ supports inserting assertions at any layers of the network.
Intuitively, it is reasonable to insert assertions for all layers throughout the network to form an integrated data sanity check. However, through our practice, it's better to select those layers that provide more representative feature patterns to insert the assertions. A widely accepted fact is that the DNN's classification functionality works in a gradually progressive manner with its computation through deeper layers\cite{zeiler2014visualizing}. In the superficial layers, DNN only learns the simple intuitionistic features from the given input, while the deeper layers synthesize the previously learning results and provide more abstract features, which are more indicative towards the final classification results. Hence, a proper selection strategy is to choose the last few layers of the DNN to insert the assertions. We believe that the outputs of these layers represent the model's deep understanding towards input data. Our practice shows that such selection leads to good performance.



On the other hand, a proper selection also improves the efficiency of the entire data sanity checking process. A complex neural network usually consists of layers at large size ({\em e.g.} the convolutional neural network(CNN)\cite{krizhevsky2012imagenet} shown in the Figure \ref{fig:method:CNN}). We can see that those superficial layers give outputs at high dimension, which require an equally high-dimensional AE network with massive neurons if assertion inserted. But through the computation of network the scale of layer output is gradually reduced({\em e.g.} via pooling layers). So deeper layers can provide compressed output with low dimension. Selecting such layers to insert assertions can avoid exhaustive computation on large AE network and therefore reduce the computation overhead.


%as introduced, our AE based assertions are applied to exploit the difference in intermediate feature pattern between valid and invalid inputs. T of the DNN's classification functionality works in a gradually progressive manner layer by layer. In the superficial layers, DNN only learns the intuitionistic features from the given input, while the deeper layers synthesize the previously learning results and provide more abstract features, which are more indicative towards the final classification results. Hence, the output of deeper layers shows more representative feature patterns.



%It's output shows condensing feature pattern with low dimension. Hence, to the efficiency concern, we only insert AE based assertions between fully connected layers. Such selection avoids exhaustive computation on large AE network, and can still achieve satisfactory performance for data sanity check as shown in experiments.

%DNN learns the complex neural network usually consists of various types of layers besides fully connected layers. {\em e.g.} the convolutional neural network(CNN)\cite{XXX} contains convolution layers and pooling layers. Such layers giving outputs at high dimension, which requires a large AE network if assertion inserted. Fortunately, fully connected layers are always a indispensable part of a neural network, which are usually placed at the end of network structure to achieve classification. 
%for deep learning system, any assertion failure indicates that the different severity level of data sanity check is required. On the one hand, a strict blocking for any suspicious invalid input is needed when applying in critical scenarios. On the other hand, it's unexpected to mistakenly reject those potential valid input in some other cases. Hence, \deep\ takes two assertion strategies, which can be flexibly adapted to detect invalid inputs in either strict or mild manner.

%We conclude the input validity verification process as Algorithm 1. Specifically, in a strict strategy, the input is rejected as an invalid input when its intermediate result fails any of the assertion check. It guarantees that for a given input, the dataflow should always follow the pre-trained feature pattern throughout its computation process. And in a mild strategy, we collect the loss from every AE based assertions, and sum them up to calculate an overall loss $L$. We check if the overall loss $L$ is under a certain threshold to determine the validity of given inputs. In this case, it permits that some layer outputs fail to satisfy the assertion constrains, but the entire computation process of the given input should not be checked as anomaly.

%Such two assertion strategies can be properly chosen according to the real situation where the deep learning system is applied. Our experiments shows that the strict strategy can detect more true positives but also collect some extra false positives. On the contrary, the result of mild strategy  contains less false positives, but it may miss some true positives. It means that the strict strategy rejects more real invalid inputs but may mistakenly reject some valid inputs as well, while the mild strategy tends to stay cautious in checking inputs as invalid and may miss some true invalid cases. Hence, a proper choice is to apply the strict strategy when system deals with critical tasks, and apply the mild strategy in other non-critical scenarios. Hence, such flexible strategies make \deep\ a high usability tool among different deep learning systems. 













==> tex/new_pre.tex <==
\section{Preliminaries} \label{sec:prelimary}

To facilitate our following discussions, we introduce some background knowledge in this section. First, we will  briefly introduce deep neural networks, as our tool focuses on DL-based systems. Then, we will show the essential functionality of AutoEncoder, which is the key underlying component of the assertion mechanism provided by \deep. 

%And lastly, we give a brief view on the concept of anomaly detection, from which the design philosophy of \deep\ is derived.


                        
\subsection{Deep Neural Network}

Deep neural network (DNN) has been proven quite effective in many application scenarios, including data analysis \cite{DBLP:journals/jbd/NajafabadiVKSWM15, DBLP:conf/icml/AndrewABL13, DBLP:conf/icml/XieGF16}, computer vision \cite{DBLP:conf/iccv/LiuLWT15, DBLP:conf/iccv/OuyangW13}, natural language processing \cite{lai2015recurrent, kim2014convolutional}.
DNN is designed as an emulation of human nervous system. It generally includes two critical activities, connection and activation. Figure \ref{fig:dnn_example} gives a classical DNN structure. It shows that DNN is organized in layers, each of which consists of multiple {\em neurons}. The general computation process of DNN follows a feed-forward manner, \emph{i.e.}, the outputs of the neurons in a layer form a vector $x$ which is sent out as an input for the connected neurons in the next layer. A neuron, specifically, is a computation unit that processes $x$ with a certain function ({\em e.g.}, linear combination $y=Wx+b$) and applies 
an activation function ({\em e.g.}, the ReLU function \cite{nair2010rectified}) of $y$ to generate its output. 
The input data of a sample, in this way, flow through the network, layer by layer, and generate a final result in the last layer. 

\begin{figure}[htbp]
	\centering
	\includegraphics[width=1\linewidth]{pic/DNN_Example.png}  
	\caption{A classical structure of deep neural network for classification.} 
	\label{fig:dnn_example}  
\end{figure}

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.9\linewidth]{pic/AutoEncoder.png}  
	\caption{Architecture of AutoEncoder} 
	\label{fig:autoencoder}  
\end{figure}
During the training phase, the final result is generally used to compute a {\em loss} value, which is minimized via certain optimization strategies.
The loss evaluates the distance between the network results and the ideal results of a target class. 
Typically, a set of properly-collected data samples are used to conduct the training process of a DNN. Its aim is to find a set of best network parameters so as to minimize the loss values for the data samples. 
This training-based nature may have its own limitation: It can only give reliable results when the input data share the similar characteristics with the training set.
\input{tex/figs/fig1.tex}


Finally, when a DNN is applied in a classification task ({\em e.g.} image classification), the number of neurons in the last layer determines how many categories the neural network can classify. 
The output of a neuron in the last layer indicates the likelihood that the input case belongs to the neuron's corresponding class. 
Generally the neuron with the largest output value is considered as that indicates the classification result, as shown in Figure \ref{fig:dnn_example}. As a result, a DNN model guarantees that every given input case will be {\em compulsively} classified into a pre-defined class, even when it actually belongs to an additional one other than those indicated by the output neurons. Unexpected system behavior may occur consequently. In this paper, we propose \deep\ to address this issue: \deep\ conducts a data sanity check to indicate that whether an input case belongs to other untrained classes. We find that such a mechanism can significantly enhance the reliability of DL-based systems. 


\subsection{Auto-Encoder}

Auto-Encoder (AE) is a kind of specific-tailored neural network capable of restoring the input data\cite{hinton2006reducing}. Figure \ref{fig:autoencoder} presents a sample architecture of the AutoEncoder. Generally, it shares a similar working process with the classic neural network described above. 
However, instead of giving classification results, such network aims at reconstructing an output vector that is similar towards the input vector
({\em i.e.} serving as a fixed-point function $f(x)\approx x$).

As shown in Figure \ref{fig:autoencoder}, it's network structure is organized in a symmetric form, which can be divided into two phases. Input data are first processed through computation into compressed vectors in the encoding phase, and then reconstructed back to their original sizes in the decoding phase. AE requires that the reconstructed data should be as close to the original input data as possible. A Mean Square Error (MSE) loss \cite{allen1971mean}, which is calculated and minimized during training, is used to represent the distance between input data and the reconstructed output. A low value of MSE loss indicates that AE successfully reconstruct an output which is rather similar to the input vector through its encoding-decoding process, while a high value shows that the input cannot be properly restored.

Similar to the training process of the classic DNN described above, AE is also trained with a certain set of training data. Hence it can only properly restore the inputs staying within the same distribution of the training data set. %Unlike traditional use of AE which aims to generate a dense representation({\em i.e.} the compressed vector given by the encoding phase) for the input data, 
We adopt this notion and consider AE as an deviation detector for the intermediate date flow of a DL model, which helps to process the assertion mechanism for data sanity check.
% to calculate the MSE loss of the reconstruction to check if the input is properly restored, and in turn evaluates the deviation of input from the training set.




 

==> tex/pre.tex <==
\section{Preliminaries} \label{sec:prelimary}

To facilitate our following discussions, we introduce some background knowledge in this section. First, we will illustrate the assertion mechanism for data sanity check in traditional software development. Then, as our tool focuses on DL-based systems, we will briefly introduce deep neural networks.

%And lastly, we give a brief view on the concept of anomaly detection, from which the design philosophy of \deep\ is derived.

\subsection{Assertion based Data Sanity Check}

Data sanity check is a mechanism that examines whether the data fed to a system is those expected during the system design \cite{boritz2005practitioners}. 
%As every system has its specific-tailored functionalities targeting a certain task, the input given must satisfy the properties corresponding to the requirement of such task. 
Even though a system's  logical functionalities are properly developed, severe system failures may still occur
when undesirable input data are fed into the system\cite{DBLP:journals/tissec/CadarGPDE08, DBLP:journals/ieeesp/Oehlert05}. A proper data sanity check can help block invalid inputs and to some extent  guarantee a system to work as expected. 
%It's worth noting that such mechanism are usually designed in a lightweight manner to preserve systems' performance\cite{XXX}. It usually turns out to be a set of very brief inspections, rather than a more exhaustive round of testing.
 
Assertions, typically, have been proved to be a very effective method of data sanity check in traditional software development \cite{DBLP:journals/annals/Hoare03, DBLP:conf/sp/WagnerKCK15, DBLP:journals/ubiquity/Saha06c}. Developers develop properly-designed, system-specific conditions, and insert the checking statements of such conditions into the target system. The satisfaction of such conditions will be checked during system runtime when the system process its input data. Applied as an instant data sanity check mechanism, assertions guarantee that every conditions should be satisfied when a valid input is given. Invalid inputs can result in assertion failure on a certain assertion, which can then been identified. Figure \ref{fig:assertion} gives an example on how assertions indicates invalid inputs.

\begin{figure}[htbp]
	\centering
	\includegraphics[width=1\linewidth]{pic/assertion.png}  
	\caption{Example for assertions used to prevent invalid input for a function computing $\sqrt{\ln x}$.} 
	\label{fig:assertion}  
\end{figure}

It's worth noting that the effectiveness of assertions is strongly related to the design of conditions. Conditions are usually manually worked out according to the system internal logic and developers' understanding on system requirements. 

This paper also proposes to perform data sanity check with a  specifically-tailored assertion mechanism for DL-based systems. Unlike traditional assertions that are typically built manually, the assertion mechanism of \deep\ is based on the mechanism of deep neural networks, and generated automatically. Through evaluating the effectiveness of \deep, We confirm that the assertion based data sanity check is of great practical significance in DL-based system.
                        
\subsection{Deep Neural Network}

Deep neural network (DNN) has been proven quite effective in many application scenarios, including data analysis \cite{DBLP:journals/jbd/NajafabadiVKSWM15, DBLP:conf/icml/AndrewABL13, DBLP:conf/icml/XieGF16}, computer vision \cite{DBLP:conf/iccv/LiuLWT15, DBLP:conf/iccv/OuyangW13}, natural language processing \cite{lai2015recurrent, kim2014convolutional}.
DNN is designed as an emulation of human nervous system. It generally includes two critical activities, connection and activation. Figure \ref{fig:dnn_example} gives a classical DNN structure. It shows that DNN is organized in layers, each of which consists of multiple {\em neurons}. The general computation process of DNN follows a feed-forward manner, \emph{i.e.}, the outputs of the neurons in a layer form a vector $x$ which is sent out as an input for the connected neurons in the next layer. A neuron, specifically, is a computation unit that processes $x$ with a certain function ({\em e.g.}, linear combination $y=Wx+b$) and applies 
an activation function ({\em e.g.}, the ReLU function \cite{nair2010rectified}) of $y$ to generate its output. 
The input data of a sample, in this way, flow through the network, layer by layer, and generate a final result in the last layer. 

\begin{figure}[htbp]
	\centering
	\includegraphics[width=1\linewidth]{pic/DNN_Example.png}  
	\caption{A classical structure of deep neural network for classification.} 
	\label{fig:dnn_example}  
\end{figure}

During the training phase, the final result is generally used to compute a {\em loss} value, which is minimized via certain optimization strategies.
The loss evaluates the distance between the network results and the ideal results of a target class. 
Typically, a set of properly-collected data samples are used to conduct the training process of a DNN. Its aim is to find a set of best network parameters so as to minimize the loss values for the data samples. 
This training-based nature may have its own limitation: It can only perform well when the input data share the similar characteristics with the training set.
\input{tex/figs/fig1.tex}


Finally, when a DNN is applied in a classification task ({\em e.g.} image classification), the number of neurons in the last layer determines how many categories the neural network can classify. 
The output of a neuron in the last layer indicates the likelihood that the input case belongs to the neuron's corresponding class. 
Generally the neuron with the largest output value is considered as that indicates the classification result, as shown in Figure \ref{fig:dnn_example}. As a result, a DNN model guarantees that every given input case will be {\em compulsively} classified into a pre-defined class, even when it actually belongs to an additional one other than those indicated by the output neurons. Unexpected system behavior may occur consequently. In this paper, we propose \deep\ to address this issue: \deep\ conducts a data sanity check to indicate that whether an input case belongs to other untrained classes. We find that such a mechanism can significantly enhance the reliability of DL-based systems. 

 
